(Seemingly) Impossible Theorems in Constructive Mathematics

We prove some constructive results that on first and maybe even on second glance seem impossible.

==> base.tex <==
\usepackage[utf8]{inputenc}

\RequirePackage[orthodox]{nag}
\usepackage{microtype}
\usepackage{booktabs}
\usepackage{mathptmx} 
\usepackage{mathtools}
\usepackage{amssymb}
\usepackage{amsthm}

%\usepackage{enumerate}
\usepackage{nicefrac}
\usepackage{xspace}
\usepackage{xcolor}
\definecolor{mylightblue}{rgb}{0.93,0.95,1.0}
\definecolor{blueish}{RGB}{71,98,168}

\usepackage{tikz}
\usetikzlibrary{external}
\usetikzlibrary{calc}
\usepackage[framemethod=TikZ]{mdframed} 

\usepackage{stmaryrd}
\usepackage{algpseudocode}
\usepackage{hyperref}
\usepackage{todonotes}
\usepackage{pifont}
\newcommand{\cmark}{\ding{51}}%
\newcommand{\xmark}{\ding{55}}%

\allowdisplaybreaks


\theoremstyle{plain}
\newtheorem{Thm}{Theorem}
\newtheorem{Theorem}[Thm]{Theorem}
\newtheorem{Remark}[Thm]{Remark}
\newtheorem{Example}[Thm]{Example}
\newtheorem{Corollary}[Thm]{Corollary}
\newtheorem{Lemma}[Thm]{Lemma}
\newtheorem{Proposition}[Thm]{Proposition}
\newtheorem{Rmk}[Thm]{Remark}
\newtheorem{Exm}[Thm]{Example}
\newtheorem{Cor}[Thm]{Corollary}
\newtheorem{Lem}[Thm]{Lemma}
\newtheorem{Pro}[Thm]{Proposition}
\newtheorem{Qu}{Question}
\newtheorem{Conj}{Conjecture}

\newtheorem{Conjecture}{Conjecture}


\theoremstyle{definition}
\newtheorem{Def}[Thm]{Definition}
\newtheorem{Definition}[Thm]{Definition}


\newcommand{\CC}{\mathcal{C}}
\newcommand{\UU}{\mathcal{U}}
\newcommand{\NN}{\mathbb{N}}
\newcommand{\RR}{\mathbb{R}}
\newcommand{\QQ}{\mathbb{Q}}
\DeclareMathOperator{\id}{\mathrm{id}}
\newcommand{\AWWKL}{\textrm{Anti-WWKL}\xspace}
\newcommand{\AFAN}{\textrm{Anti-FAN}\xspace}
\newcommand{\FAN}{\textrm{FAN}}
\newcommand{\FAND}{\textrm{FAN}\texorpdfstring{\ensuremath{_{\Delta}}\xspace}{∆}}
\newcommand{\FANP}{\textrm{FAN}\texorpdfstring{\ensuremath{_{\Pi^{0}_{1}}}\xspace}{Π-0-1}}
\newcommand{\FANc}{\textrm{FAN}\texorpdfstring{\ensuremath{_{c}}\xspace}{c}}
\newcommand{\FANst}{\texorpdfstring{\textrm{FAN}\ensuremath{_{\textrm{stable}}}\xspace}{FAN-stable}}
\newcommand{\FANf}{\texorpdfstring{\textrm{FAN}\ensuremath{_{\textrm{full}}}\xspace}{FAN-full}}
\newcommand{\BDN}{\textrm{BD-N}\xspace}
\newcommand{\wBDN}{\textrm{wBD-N}\xspace}
\newcommand{\LEM}{\hyperref[PR:LEM]{\textrm{LEM}}\xspace}
\newcommand{\WLEM}{\hyperref[PR:WLEM]{\textrm{WLEM}}\xspace}

\newcommand{\LLPO}{\hyperref[PR:LLPO]{\textrm{LLPO}}\xspace}
\newcommand{\LLPOn}[1]{\texorpdfstring{\ensuremath{\textrm{LLPO}_{#1}}\xspace}{LLPOn}}
\newcommand{\WLPO}{\texorpdfstring{\hyperref[PR:WLPO]{\textrm{WLPO}}\xspace}{WLPO}}
\newcommand{\LPO}{\hyperref[PR:LPO]{\textrm{LPO}}\xspace}
\newcommand{\nWLPO}{\texorpdfstring{\ensuremath{\neg\textrm{WLPO}}\xspace}{¬WLPO}}
\newcommand{\nLPO}{\texorpdfstring{\ensuremath{\neg\textrm{LPO}}\xspace}{¬LPO}}
\newcommand{\WKL}{\hyperref[PR:WKL]{\textrm{WKL}}\xspace}
\newcommand{\WKLpp}{\textrm{WKL!!}\xspace}

\newcommand{\WKLp}[1]{\texorpdfstring{\ensuremath{\textrm{WKL}^{\prime}(#1)}\xspace}{'}}
\newcommand{\WWKL}{\textrm{WWKL}\xspace}
\newcommand{\UCT}{\textrm{UCT}\xspace}
\newcommand{\KT}{\textrm{KT}\xspace}
\renewcommand{\SS}{\textrm{SS}\xspace}
\newcommand{\iSS}{\textrm{iSS}\xspace}
\newcommand{\KTs}[1]{\ensuremath{\textrm{KTs}(#1)}\xspace}
\newcommand{\AS}[2]{\hyperref[PR:AS]{\ensuremath{\textrm{AS}_{#1}^{\, #2}}}}
\newcommand{\MPv}{\texorpdfstring{\ensuremath{\hyperref[PR:MPv]{\textrm{MP}^{\vee}}}\xspace}{MPv}}
\newcommand{\MP}{\hyperref[PR:MP]{\textrm{MP}}\xspace}
\newcommand{\WMP}{\hyperref[PR:WMP]{\textrm{WMP}}\xspace}
\newcommand{\WPFP}{\textrm{WPFP}\xspace}
\newcommand{\PFP}{\textrm{PFP}\xspace}
\newcommand{\KS}{\textrm{KS}\xspace}
\newcommand{\OI}[1]{\texorpdfstring{\textrm{OI}{\ensuremath{(#1)}}\xspace}{OI}}
\newcommand{\BID}{\texorpdfstring{\textrm{BI}{\ensuremath{_{\Delta}}}\xspace}{BI{∆}}}
\newcommand{\BIM}{\texorpdfstring{\textrm{BI}{\ensuremath{_{M}}}\xspace}{BIM}}
\newcommand{\BI}{\textrm{BI}}
\newcommand{\UZS}{\textrm{UZS}\xspace}
\newcommand{\UUZS}{\textrm{UUZS}\xspace}
\newcommand{\POS}{\textrm{POS}\xspace}


\newcommand{\define}[1]{\emph{#1}}


\renewcommand{\mid}{\, \middle| \,}
\newcommand{\menge}[1]{\ensuremath{\left\{ #1 \right\}}}
\newcommand{\set}[2]{\mbox{\ensuremath{\left\{ \,#1 \mid #2 \,\right\}}}}

\newcommand{\ext}[1]{\llbracket #1  \rrbracket}
\newcommand{\fa}[2]{\forall {#1} : {#2}}
\newcommand{\ex}[2]{\exists {#1} : {#2}}
\newcommand{\Interior}[1]{\mathrm{Int}\left(#1\right)}
\newcommand{\Closure}[1]{\overline{#1}}
\newcommand{\Complement}[1]{{#1}^\prime}
\DeclarePairedDelimiter{\abs}{\lvert}{\rvert}
\DeclarePairedDelimiter{\norm*}{\lVert}{\rVert}
\DeclarePairedDelimiter{\bracks}{\lbrack}{\rbrack}


\newcommand{\co}{\colon\!}
\newcommand{\CS}{2^{\NN}}
\newcommand{\cS}{2^{\ast}}
\newcommand{\BS}{\NN^{\NN}}
\newcommand{\Ninf}{\NN_{\infty}}

